Expanded Comprehensive Robotic Cholecystectomy Dataset (CRCD)

In recent years, the application of machine learning to minimally invasive surgery (MIS) has attracted considerable interest. Datasets are critical to the use of such techniques. This paper presents a unique dataset recorded during ex vivo pseudo-cholecystectomy procedures on pig livers using the da Vinci Research Kit (dVRK). Unlike existing datasets, it addresses a critical gap by providing comprehensive kinematic data, recordings of all pedal inputs, and offers a time-stamped record of the endoscope's movements. This expanded version also includes segmentation and keypoint annotations of images, enhancing its utility for computer vision applications. Contributed by seven surgeons with varied backgrounds and experience levels that are provided as a part of this expanded version, the dataset is an important new resource for surgical robotics research. It enables the development of advanced methods for evaluating surgeon skills, tools for providing better context awareness, and automation of surgical tasks. Our work overcomes the limitations of incomplete recordings and imprecise kinematic data found in other datasets. To demonstrate the potential of the dataset for advancing automation in surgical robotics, we introduce two models that predict clutch usage and camera activation, a 3D scene reconstruction example, and the results from our keypoint and segmentation models.

==> tables/surgeon_background.tex <==
\begin{tablehere}
\centering
\resizebox{\columnwidth}{!}{%
\begin{tabular}{c|c|c}

\hline
\hline
         \textbf{Surgeon}    & \textbf{Number of procedures} & \textbf{Additional Information} \\ \hline
\textbf{A}   & -                  & 3              \\
\textbf{B}   & 1500                  & -              \\
\textbf{C}   & -                 & -              \\
\textbf{D}   & 65                  & -              \\
\textbf{E}   & -                  & -              \\
\textbf{F}   & -                  & -              \\
\textbf{G}   & 1000                  & -              \\  
\hline
\hline
\end{tabular}}
\caption{Surgeons background provided with the dataset}
\label{tab:surgdata}
\vspace{-5mm}
\end{tablehere}  


==> tables/table_calibration.tex <==
\begin{tablehere}[t]

\begin{tabular}{l|l|l}
\hline
\hline
\textbf{Measure (distance)}          & \textbf{dVRK $\Leftrightarrow$ ArUco }     & \textbf{Custom $\Leftrightarrow$ ArUco} \\ \hline

\multirow{3}{*}{Mean Error}          &X: $11.0mm$                                &X: $5.6mm$                               \\
                                     &Y: $50.1mm$                                &Y: $2.5mm$                               \\
                                     &Z: $20.9mm$                                &Z: $1.1mm$                               \\ \hline
\multirow{3}{*}{Standard deviation}  &X: $4.9mm$                                &X: $3.6mm$                               \\
                                     &Y: $2.0mm$                                &Y: $2.1mm$                               \\
                                     &Z: $3.9mm$                                &Z: $2.2mm$                               \\
\hline
\hline
\end{tabular}%

\caption{The first Row shows the distance between the kinematics data obtained by dVRK compared to the one obtained by detecting the ArUco markers, while the second row shows the distance between the kinematics data by our custom calibration compared to the one obtained by detecting the ArUco markers. We can observe that the mean error decreases drastically (a factor of 1.96 for X, 20.04 for Y, and 19 for Z). }
\label{tab:calib_table}
\vspace{-7mm}
\end{tablehere}

==> tables/table_dataset.tex <==


% % \begin{sidewaystable*}[t]
% \begin{tablehere}[t]

% \centering
% \renewcommand{\arraystretch}{1.5}
% \resizebox{\columnwidth}{!}{%
% \begin{tabular}{l|c|c|c}
% \hline
% \hline
% \textbf{Type} & \textbf{Features} & \textbf{Dim} & \textbf{Description (Units)} \\ \hline
% \multirow{3}{*}{\textbf{ECM}}       & Endoscope Tip Cartesian Pose         & 7       & Translation \{$x$, $y$, $z$\} (m), Quaternion \{$x$, $y$, $z$, $w$\} (rad) \\ \cline{2-4}
%                                     & Local Endoscope Tip Cartesian Pose   & 7       & Translation \{$x$, $y$, $z$\} (m), Quaternion \{$x$, $y$, $z$, $w$\} (rad) \\ \cline{2-4}
%                                     & Arm Joint State                      & 12      & Joint Position \{$\theta(4)$\} (rad), Joint Velocity \{$\dot{\theta}(4)$\} (rad/s), Joint Effort \{$\tau(4)$\} (N) \\ \hline
                                    
% \multirow{4}{*}{\textbf{MTML}}      & Manipulator Tip Cartesian Pose       & 7       & Translation \{$x$, $y$, $z$\} (m), Quaternion \{$x$, $y$, $z$, $w$\} (rad) \\ \cline{2-4}
%                                     & Local Manipulator Tip Cartesian Pose & 7       & Translation \{$x$, $y$, $z$\} (m), Quaternion \{$x$, $y$, $z$, $w$\} (rad) \\ \cline{2-4}
%                                     & Manipulator Joint State              & 18      & Joint Position \{$\theta(6)$\} (rad), Joint Velocity \{$\dot{\theta}(6)$\} (rad/s), Joint Effort \{$\tau(6)$\} (N) \\ \cline{2-4}
%                                     & Manipulator Gripper Joint State      & 1       & Joint Position \{$\theta(1)$\} (rad) \\ \hline
                                    
% \multirow{4}{*}{\textbf{MTMR}}      & Manipulator Tip Cartesian Pose       & 7       & Translation \{$x$, $y$, $z$\} (m), Quaternion \{$x$, $y$, $z$, $w$\} (rad) \\ \cline{2-4}
%                                     & Local Manipulator Tip Cartesian Pose & 7       & Translation \{$x$, $y$, $z$\} (m), Quaternion \{$x$, $y$, $z$, $w$\} (rad) \\ \cline{2-4}
%                                     & Manipulator Joint State              & 18      & Joint Position \{$\theta(6)$\} (rad), Joint Velocity \{$\dot{\theta}(6)$\} (rad/s), Joint Effort \{$\tau(6)$\} (N) \\ \cline{2-4}
%                                     & Manipulator Gripper Joint State      & 1       & Joint Position \{$\theta(1)$\} (rad) \\ \hline
                                    
% \multirow{4}{*}{\textbf{PSM1}}      & Instrument Tip Cartesian Pose        & 7       & Translation \{$x$, $y$, $z$\} (m), Quaternion \{$x$, $y$, $z$, $w$\} (rad) \\ \cline{2-4}
%                                     & Local Instrument Tip Cartesian Pose  & 7       & Translation \{$x$, $y$, $z$\} (m), Quaternion \{$x$, $y$, $z$, $w$\} (rad) \\ \cline{2-4}
%                                     & Arm Joint State                      & 18      & Joint Position \{$\theta(6)$\} (rad), Joint Velocity \{$\dot{\theta}(6)$\} (rad/s), Joint Effort \{$\tau(6)$\} (N) \\ \cline{2-4}
%                                     & Instrument Tip Jaw Joint State       & 3       & Joint Position \{$\theta(1)$\} (rad), Joint Velocity \{$\dot{\theta}(1)$\} (rad/s), Joint Effort \{$\tau(1)$\} (N) \\ \hline
                                    
% \multirow{4}{*}{\textbf{PSM2}}      & Instrument Tip Cartesian Pose        & 7       & Translation \{$x$, $y$, $z$\} (m), Quaternion \{$x$, $y$, $z$, $w$\} (rad) \\ \cline{2-4}
%                                     & Local Instrument Tip Cartesian Pose  & 7       & Translation \{$x$, $y$, $z$\} (m), Quaternion \{$x$, $y$, $z$, $w$\} (rad) \\ \cline{2-4}
%                                     & Arm Joint State                      & 18      & Joint Position \{$\theta(6)$\} (rad), Joint Velocity \{$\dot{\theta}(6)$\} (rad/s), Joint Effort \{$\tau(6)$\} (N) \\ \cline{2-4}
%                                     & Instrument Tip Jaw Joint State       & 3       & Joint Position \{$\theta(1)$\} (rad), Joint Velocity \{$\dot{\theta}(1)$\} (rad/s), Joint Effort \{$\tau(1)$\} (N) \\ \hline \hline
% \multirow{3}{*}{\textbf{Pedals}}    & Clutch Pedal State                  & 1       & Boolean (True when activated, False otherwise)  \\ \cline{2-4}
%                                     & Camera Pedal State                  & 1       & Boolean (True when activated, False otherwise) \\ \cline{2-4}
%                                     & Monopolar Pedal State               & 1       & Boolean (False when activated, True otherwise) \\
% \hline
% \hline
% \end{tabular}}
% \caption{List of kinematic variables including the pedal signals. ``Local'' tip cartesian pose relates the position of the arm's tip to the arm's base frame (e.g. $g_{rt}$ of the PSM). Otherwise, it is the pose of the arm's tip to its reference frame (the Helper frame, ECM tip frame, and HRSV frame for ECM, PSMs, and MTMs respectively).}
% \label{tab:feature_set_signals}
% \vspace{-3mm}
% % \end{sidewaystable*}
% \end{tablehere}
\begin{table*}[t]
\centering
\renewcommand{\arraystretch}{1.5}
\resizebox{\textwidth}{!}{%
\begin{tabular}{l|c|c|c}
\hline
\hline
\textbf{Type} & \textbf{Features} & \textbf{Dim} & \textbf{Description (Units)} \\ \hline
\multirow{3}{*}{\textbf{ECM}}       & Endoscope Tip Cartesian Pose         & 7       & Translation \{$x$, $y$, $z$\} (m), Quaternion \{$x$, $y$, $z$, $w$\} (rad) \\ \cline{2-4}
                                    & Local Endoscope Tip Cartesian Pose   & 7       & Translation \{$x$, $y$, $z$\} (m), Quaternion \{$x$, $y$, $z$, $w$\} (rad) \\ \cline{2-4}
                                    & Arm Joint State                      & 12      & Joint Position \{$\theta(4)$\} (rad), Joint Velocity \{$\dot{\theta}(4)$\} (rad/s), Joint Effort \{$\tau(4)$\} (N) \\ \hline
                                    
\multirow{4}{*}{\textbf{MTML}}      & Manipulator Tip Cartesian Pose       & 7       & Translation \{$x$, $y$, $z$\} (m), Quaternion \{$x$, $y$, $z$, $w$\} (rad) \\ \cline{2-4}
                                    & Local Manipulator Tip Cartesian Pose & 7       & Translation \{$x$, $y$, $z$\} (m), Quaternion \{$x$, $y$, $z$, $w$\} (rad) \\ \cline{2-4}
                                    & Manipulator Joint State              & 18      & Joint Position \{$\theta(6)$\} (rad), Joint Velocity \{$\dot{\theta}(6)$\} (rad/s), Joint Effort \{$\tau(6)$\} (N) \\ \cline{2-4}
                                    & Manipulator Gripper Joint State      & 1       & Joint Position \{$\theta(1)$\} (rad) \\ \hline
                                    
\multirow{4}{*}{\textbf{MTMR}}      & Manipulator Tip Cartesian Pose       & 7       & Translation \{$x$, $y$, $z$\} (m), Quaternion \{$x$, $y$, $z$, $w$\} (rad) \\ \cline{2-4}
                                    & Local Manipulator Tip Cartesian Pose & 7       & Translation \{$x$, $y$, $z$\} (m), Quaternion \{$x$, $y$, $z$, $w$\} (rad) \\ \cline{2-4}
                                    & Manipulator Joint State              & 18      & Joint Position \{$\theta(6)$\} (rad), Joint Velocity \{$\dot{\theta}(6)$\} (rad/s), Joint Effort \{$\tau(6)$\} (N) \\ \cline{2-4}
                                    & Manipulator Gripper Joint State      & 1       & Joint Position \{$\theta(1)$\} (rad) \\ \hline
                                    
\multirow{4}{*}{\textbf{PSM1}}      & Instrument Tip Cartesian Pose        & 7       & Translation \{$x$, $y$, $z$\} (m), Quaternion \{$x$, $y$, $z$, $w$\} (rad) \\ \cline{2-4}
                                    & Local Instrument Tip Cartesian Pose  & 7       & Translation \{$x$, $y$, $z$\} (m), Quaternion \{$x$, $y$, $z$, $w$\} (rad) \\ \cline{2-4}
                                    & Arm Joint State                      & 18      & Joint Position \{$\theta(6)$\} (rad), Joint Velocity \{$\dot{\theta}(6)$\} (rad/s), Joint Effort \{$\tau(6)$\} (N) \\ \cline{2-4}
                                    & Instrument Tip Jaw Joint State       & 3       & Joint Position \{$\theta(1)$\} (rad), Joint Velocity \{$\dot{\theta}(1)$\} (rad/s), Joint Effort \{$\tau(1)$\} (N) \\ \hline
                                    
\multirow{4}{*}{\textbf{PSM2}}      & Instrument Tip Cartesian Pose        & 7       & Translation \{$x$, $y$, $z$\} (m), Quaternion \{$x$, $y$, $z$, $w$\} (rad) \\ \cline{2-4}
                                    & Local Instrument Tip Cartesian Pose  & 7       & Translation \{$x$, $y$, $z$\} (m), Quaternion \{$x$, $y$, $z$, $w$\} (rad) \\ \cline{2-4}
                                    & Arm Joint State                      & 18      & Joint Position \{$\theta(6)$\} (rad), Joint Velocity \{$\dot{\theta}(6)$\} (rad/s), Joint Effort \{$\tau(6)$\} (N) \\ \cline{2-4}
                                    & Instrument Tip Jaw Joint State       & 3       & Joint Position \{$\theta(1)$\} (rad), Joint Velocity \{$\dot{\theta}(1)$\} (rad/s), Joint Effort \{$\tau(1)$\} (N) \\ \hline \hline
\multirow{3}{*}{\textbf{Pedals}}    & Clutch Pedal State                  & 1       & Boolean (True when activated, False otherwise)  \\ \cline{2-4}
                                    & Camera Pedal State                  & 1       & Boolean (True when activated, False otherwise) \\ \cline{2-4}
                                    & Monopolar Pedal State               & 1       & Boolean (False when activated, True otherwise) \\
\hline
\hline
\end{tabular}}
\caption{List of kinematic variables including the pedal signals. ``Local'' tip cartesian pose relates the position of the arm's tip to the arm's base frame (e.g. $g_{rt}$ of the PSM). Otherwise, it is the pose of the arm's tip to its reference frame (the Helper frame, ECM tip frame, and HRSV frame for ECM, PSMs, and MTMs respectively).}
\label{tab:feature_set_signals}
\vspace{-3mm}
\end{table*}

